Optimizing Mode Connectivity via Neuron Alignment

The loss landscapes of deep neural networks are not well understood due to their high nonconvexity. Empirically, the local minima of these loss functions can be connected by a learned curve in model space, along which the loss remains nearly constant; a feature known as mode connectivity. Yet, current curve finding algorithms do not consider the influence of symmetry in the loss surface created by model weight permutations. We propose a more general framework to investigate the effect of symmetry on landscape connectivity by accounting for the weight permutations of the networks being connected. To approximate the optimal permutation, we introduce an inexpensive heuristic referred to as neuron alignment. Neuron alignment promotes similarity between the distribution of intermediate activations of models along the curve. We provide theoretical analysis establishing the benefit of alignment to mode connectivity based on this simple heuristic. We empirically verify that the permutation given by alignment is locally optimal via a proximal alternating minimization scheme. Empirically, optimizing the weight permutation is critical for efficiently learning a simple, planar, low-loss curve between networks that successfully generalizes. Our alignment method can significantly alleviate the recently identified robust loss barrier on the path connecting two adversarial robust models and find more robust and accurate models on the path.

==> extra.tex <==
\begin{table*}[htb]
    \caption{Accuracy of model ensembles constructed from the curve connecting trained models on the CIFAR100 dataset. Standard deviation is reported as well. All ensembles function by averaging the predictions of their component models. The curve ensembles are constructed by sampling the curve at the values of $t$ listed. The independent ensemble consists of three independently trained models.}
    \label{tab:ensembling}
    \centering
    \begin{tabular}{|c|r r r|r|r|}
        \hline
        & \multicolumn{3}{c|}{Curve Ensembles (\%)} & \multirow{3}{6em}{Independent Ensembles (\%)} & \multirow{3}{5em}{Individual Models}\\
        curve parameter $t$ & \{0.0, 1.0\} & \multicolumn{2}{c|}{\{0.0, 0.5, 1.0\}} & & \\
         &  & Unaligned & Aligned & & \\
        \hline 
        TinySix & $41.80 \pm 0.15$ & $42.66 \pm 0.48$ & $\mathbf{43.82 \pm 0.78}$ & $42.05 \pm 0.26$ & $40.10 \pm 0.30$\\
        \hline
        TinyTen & $61.23 \pm 0.36$ & $61.39 \pm 0.25$ & $\mathbf{62.40 \pm 0.30}$ & $61.76 \pm 0.01$ & $58.10 \pm 0.50$ \\
        \hline
        ResNet32  & $71.35 \pm 0.30$ & $72.13 \pm 0.12$ & $\mathbf{72.33 \pm 0.12}$ & $72.03 \pm 0.08$ & $67.10 \pm 0.50$\\
        \hline
        VGG16 & $74.00 \pm 0.17$ & $74.69 \pm 0.22$ & $\mathbf{74.91 \pm 0.10}$ & $74.88 \pm 0.06$ & $70.90 \pm 0.30$\\
        \hline
    \end{tabular}
\end{table*}
